Understanding Skills for OSS Communities on GitHub

The development of open source software (OSS) is a broad field which requires diverse skill sets. For example, maintainers help lead the project and promote its longevity, technical writers assist with documentation, bug reporters identify defects in software, and developers program the software. However, it is unknown which skills are used in OSS development as well as OSS contributors' general attitudes towards skills in OSS. In this paper, we address this gap by administering a survey to a diverse set of 455 OSS contributors. Guided by these responses as well as prior literature on software development expertise and social factors of OSS, we develop a model of skills in OSS that considers the many contexts OSS contributors work in. This model has 45 skills in the following 9 categories: technical skills, working styles, problem solving, contribution types, project-specific skills, interpersonal skills, external relations, management, and characteristics. Through a mix of qualitative and quantitative analyses, we find that OSS contributors are actively motivated to improve skills and perceive many benefits in sharing their skills with others. We then use this analysis to derive a set of design implications and best practices for those who incorporate skills into OSS tools and platforms, such as GitHub.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.
	       

==> lookup_participants.tex <==
\lookupPut{R_Abq2BR9gBTsujAZ}{P1}
\lookupPut{R_3QJmczfVmsX0R6K}{P2}
\lookupPut{R_1M3Nsv6Af2bR7rS}{P3}
\lookupPut{R_p9FY9CK3d5ODp4d}{P4}
\lookupPut{R_25t1KSlmYEvXaOF}{P5}
\lookupPut{R_3R8HLrFa6xH58cX}{P6}
\lookupPut{R_1LUsQfHdoxpX3FW}{P7}
\lookupPut{R_NVLasmamWQ3THX3}{P8}
\lookupPut{R_0VfDxpBwEmZxlcJ}{P9}
\lookupPut{R_2CV87PJRcFAP2T2}{P10}
\lookupPut{R_1Dx3r6WzVHrFK3i}{P11}
\lookupPut{R_1obYzQ8epn0YA1T}{P12}
\lookupPut{R_11jCVe7qHCuOCcW}{P13}
\lookupPut{R_pufhod4gYrc6Z9v}{P14}
\lookupPut{R_33x8RNYTqEDBsdI}{P15}
\lookupPut{R_3lVOwui1uqPUXda}{P16}
\lookupPut{R_2ebDHyFiVXPr8Qh}{P17}
\lookupPut{R_2zC5ofuQV0viNST}{P18}
\lookupPut{R_2Pjuj3Fct4EzogS}{P19}
\lookupPut{R_u7wRN7nn7XfOsA9}{P20}
\lookupPut{R_ueqaZw19SrAK83D}{P21}
\lookupPut{R_1QskZirgKCsUo7U}{P22}
\lookupPut{R_3EGwwhVvIeiQyNW}{P23}
\lookupPut{R_29nXl92y6rCPciO}{P24}
\lookupPut{R_tJrQIk6s1eEnZC1}{P25}
\lookupPut{R_R4iIExSzKei6yjv}{P26}
\lookupPut{R_1k1Bok5F3AoYMZ3}{P27}
\lookupPut{R_1gGCOOLcJqtNb1C}{P28}
\lookupPut{R_tDnYbecmCAS03gB}{P29}
\lookupPut{R_3iDAXY6BpO1sthX}{P30}
\lookupPut{R_32PXCJs51BmEE4p}{P31}
\lookupPut{R_R8khgvz3arN4oiB}{P32}
\lookupPut{R_30ppIgogNTC4q3u}{P33}
\lookupPut{R_1eFv96abv8vhPnZ}{P34}
\lookupPut{R_1q1AWLuBoMsbmi2}{P35}
\lookupPut{R_2fjISaqIumpMFLj}{P36}
\lookupPut{R_3hb6drwx6gPMg7d}{P37}
\lookupPut{R_2ceI8mcZhuQoAQM}{P38}
\lookupPut{R_23UGcAXkTnHWvpi}{P39}
\lookupPut{R_u941XGUoCwKgMo1}{P40}
\lookupPut{R_3iJWTXGCQATu4Pj}{P41}
\lookupPut{R_3NSV983iR4WPiXn}{P42}
\lookupPut{R_RIbA9JTcOqm6tvb}{P43}
\lookupPut{R_2zT3HOKdHV4EuVU}{P44}
\lookupPut{R_2P6wPRiDXkV7A0f}{P45}
\lookupPut{R_2PvCf4o70wAU5VU}{P46}
\lookupPut{R_3kHyMkFpcgxKmf0}{P47}
\lookupPut{R_pDC1DMUXAJJw3UB}{P48}
\lookupPut{R_10wrM2WdlA5Qo0R}{P49}
\lookupPut{R_1q9BpDZg9VgPsBZ}{P50}
\lookupPut{R_6SiNXH8DmuBErvP}{P51}
\lookupPut{R_277l4pW66mQbBHO}{P52}
\lookupPut{R_2cu1ZcPxuTLDizl}{P53}
\lookupPut{R_2f0N885ybxfC9gx}{P54}
\lookupPut{R_3CBOk54KYzln35s}{P55}
\lookupPut{R_1g5e4eYEPY4JC3j}{P56}
\lookupPut{R_2S17RpEEewNiwkJ}{P57}
\lookupPut{R_2tMty22IqpCKjnC}{P58}
\lookupPut{R_Rz670qsfKbhTj8Z}{P59}
\lookupPut{R_2B9E6rqUy7Pz0iL}{P60}
\lookupPut{R_1r7WQAUogie64bW}{P61}
\lookupPut{R_3gRdVOAnby137X6}{P62}
\lookupPut{R_SCc3CQtdCMzgKNH}{P63}
\lookupPut{R_eqR2iiJoMo4Calz}{P64}
\lookupPut{R_31tvWn9Ve6tws4K}{P65}
\lookupPut{R_1LST4zI6vvQVCZX}{P66}
\lookupPut{R_29jqIQhEE6FJPiv}{P67}
\lookupPut{R_1NbuKQTuQvOQ7K0}{P68}
\lookupPut{R_41MLZXd8lD21XoZ}{P69}
\lookupPut{R_V4hoGzO0spWejgR}{P70}
\lookupPut{R_3lWbGsBabOaAv35}{P71}
\lookupPut{R_tDv2gSPk10nv92p}{P72}
\lookupPut{R_1msf9EuMNd7cJ6x}{P73}
\lookupPut{R_3dS8kc3qA5yIYTj}{P74}
\lookupPut{R_1OlPf5si0Lb7tpx}{P75}
\lookupPut{R_20UarHA5QwiEaOr}{P76}
\lookupPut{R_55f82yM2K6PylC9}{P77}
\lookupPut{R_2fcYeZgH7RcMOn9}{P78}
\lookupPut{R_1jPVQb4EY7kGOUS}{P79}
\lookupPut{R_1rIW30NO2WuBtLY}{P80}
\lookupPut{R_1BPDa9eko1khrlx}{P81}
\lookupPut{R_2aD1cpjt4R3Olyz}{P82}
\lookupPut{R_28MS4Ld3m7MWhSf}{P83}
\lookupPut{R_3pcgTSCg5rGQRSg}{P84}
\lookupPut{R_yPWocG4W3O0nKVz}{P85}
\lookupPut{R_325vbTjWO6Hd7jy}{P86}
\lookupPut{R_1i3tmQc6TSQHCr0}{P87}
\lookupPut{R_3qvr0tsI49OTFD6}{P88}
\lookupPut{R_1hQlBSQnjYZJJes}{P89}
\lookupPut{R_31mgQ8F0MJik57G}{P90}
\lookupPut{R_3h6dw6lET34xrMj}{P91}
\lookupPut{R_1dgllrGZfoHxdgu}{P92}
\lookupPut{R_1k0UuDfbnkWjPMo}{P93}
\lookupPut{R_cSa7jCmVMjS54kN}{P94}
\lookupPut{R_vAmd1vZVRFfbkEV}{P95}
\lookupPut{R_2B9jRvNxtZolwf0}{P96}
\lookupPut{R_2TYQO6oJiQp4eoX}{P97}
\lookupPut{R_syPd2BxVfac0TIJ}{P98}
\lookupPut{R_1eFY3p7Cdr3ajx8}{P99}
\lookupPut{R_2EtIPwvuROQL3gb}{P100}
\lookupPut{R_3NUw6ECSwMN030U}{P101}
\lookupPut{R_2zcDkCsMuQq6aSZ}{P102}
\lookupPut{R_1IvhUoPCxR8e2se}{P103}
\lookupPut{R_bILuxUoouglKL5v}{P104}
\lookupPut{R_3snR3zX6LOBxkpl}{P105}
\lookupPut{R_1OCRRxR4kK5PxbS}{P106}
\lookupPut{R_VIi801054My3Ygp}{P107}
\lookupPut{R_8tRvEGAQMvN2EYF}{P108}
\lookupPut{R_2WUwrfaJeCipTLr}{P109}
\lookupPut{R_UA5tdbFdLAOI5EJ}{P110}
\lookupPut{R_2SrwjHpPjTFENdK}{P111}
\lookupPut{R_2ZULSQNOYmrAm0r}{P112}
\lookupPut{R_XGL2exJfm8mKPbb}{P113}
\lookupPut{R_24qv3KbVmXGLTUE}{P114}
\lookupPut{R_2f731eMh6jUJcUu}{P115}
\lookupPut{R_2zcrg66yY5pW8MO}{P116}
\lookupPut{R_BzjAhqytp2OUHER}{P117}
\lookupPut{R_2yscD6FQNJLFQcq}{P118}
\lookupPut{R_29akWqbimizCeAQ}{P119}
\lookupPut{R_1IL8IWJZG4KmMIQ}{P120}
\lookupPut{R_1mfO2yqSPTNpeLD}{P121}
\lookupPut{R_XnPJInpbKajT8pb}{P122}
\lookupPut{R_3dROkdargf7Tb9m}{P123}
\lookupPut{R_3KrsWpWtDWZXY94}{P124}
\lookupPut{R_UcnlaWPisAkkSHf}{P125}
\lookupPut{R_1jGSugYj25gFfAT}{P126}
\lookupPut{R_2fHibzuxby6pjI2}{P127}
\lookupPut{R_78K3k4x7t0M2PZL}{P128}
\lookupPut{R_3felyhCMdOOO4LF}{P129}
\lookupPut{R_do3dgHY0I36dVsJ}{P130}
\lookupPut{R_2zo48F8yLuPXcuR}{P131}
\lookupPut{R_2asHwgQ4hyJvf3P}{P132}
\lookupPut{R_27rjQsYrKawUaA9}{P133}
\lookupPut{R_pxWwAtfH0uPqGvD}{P134}
\lookupPut{R_32PHfk9XXghaX9F}{P135}
\lookupPut{R_WxnIMK3N7pWaYcF}{P136}
\lookupPut{R_2dsEJCtPlNFq37S}{P137}
\lookupPut{R_xGh9e2fuowtplS1}{P138}
\lookupPut{R_2wgYqQViEEIaGOV}{P139}
\lookupPut{R_Tbi3TDfCiw3cwM1}{P140}
\lookupPut{R_2BtYKiYuIs9QwAE}{P141}
\lookupPut{R_3gYM8frafAaiBlw}{P142}
\lookupPut{R_2Vqq1dsyWyZ3S4x}{P143}
\lookupPut{R_2zMZCvLBHRFtnu1}{P144}
\lookupPut{R_RC56rdhco802XPX}{P145}
\lookupPut{R_3qED5EgKAfz8lKD}{P146}
\lookupPut{R_2uVfodbMmAOhNf3}{P147}
\lookupPut{R_2xxvKL7MMDYo57A}{P148}
\lookupPut{R_3P4BQxJs29TVoxM}{P149}
\lookupPut{R_27xwVHg2HRrDxLo}{P150}
\lookupPut{R_pGJc9kMnkEOPGA9}{P151}
\lookupPut{R_39IQIZGiWqqxLIR}{P152}
\lookupPut{R_2QYwOO05QNpTli9}{P153}
\lookupPut{R_2TMNjS1J9BPDcyy}{P154}
\lookupPut{R_2VmrZDSiLB4iPZb}{P155}
\lookupPut{R_1fd7wE31tWZI8tl}{P156}
\lookupPut{R_2coxjE7kCaI0azt}{P157}
\lookupPut{R_3iJ7Wuv50Cy2Wyd}{P158}
\lookupPut{R_3J7SkAszVsIlNCk}{P159}
\lookupPut{R_3FPAjgtTItg6atj}{P160}
\lookupPut{R_2CdF2HnViuD57XI}{P161}
\lookupPut{R_3qg2VJcsRyVNeD5}{P162}
\lookupPut{R_3rSX4toa5wvGYqf}{P163}
\lookupPut{R_1NFGlbQ5rWlLVAq}{P164}
\lookupPut{R_006kDsD6rt7ZSc9}{P165}
\lookupPut{R_Rs1zYd2ILXIhS01}{P166}
\lookupPut{R_3iwNEWMVUDTROLk}{P167}
\lookupPut{R_3QF8vUqWA0CHhGu}{P168}
\lookupPut{R_2XdnMXItVT56UTh}{P169}
\lookupPut{R_XZAS92Ev0U3lDAl}{P170}
\lookupPut{R_3GBul4DfpCPEYqf}{P171}
\lookupPut{R_2AGxvCCpvU0qzAA}{P172}
\lookupPut{R_s5RAq4E4Yaa5AaZ}{P173}
\lookupPut{R_byi48vxzpzsedPP}{P174}
\lookupPut{R_12gtpgmFmk2jBS7}{P175}
\lookupPut{R_1LdI9m6Qg35LAHI}{P176}
\lookupPut{R_3emepjTnKCpeuLX}{P177}
\lookupPut{R_2t5cLsMNRMFdRiQ}{P178}
\lookupPut{R_2VDXhkSnafEfPCb}{P179}
\lookupPut{R_bBiNjRigSCr3QpX}{P180}
\lookupPut{R_1BP0LKT5rlHzgJv}{P181}
\lookupPut{R_1ddfwrg6uLmN7r4}{P182}
\lookupPut{R_1QtjQPI9SWYzWLC}{P183}
\lookupPut{R_3rP98giE9XNUmXe}{P184}
\lookupPut{R_5bwRrrm8QJXicEh}{P185}
\lookupPut{R_AL5T6oBQFjG0p6p}{P186}
\lookupPut{R_vUijTOliIth8Rqx}{P187}
\lookupPut{R_Ath7Jwsh93gQzh7}{P188}
\lookupPut{R_2ypx6KewLgzp5dY}{P189}
\lookupPut{R_3rZjNTs28sbhInE}{P190}
\lookupPut{R_xyL3YrADO1ws6yt}{P191}
\lookupPut{R_2Pb85dk8rJTNqWP}{P192}
\lookupPut{R_1gFxPw3QJ48vEso}{P193}
\lookupPut{R_2teV0aOo0jpth2X}{P194}
\lookupPut{R_2EEoOIFfgAGP9aU}{P195}
\lookupPut{R_3NKM2PXNqF6pnQ5}{P196}
\lookupPut{R_1mDEyIKrQdGR0HX}{P197}
\lookupPut{R_12Dc0LhGgF7kKP6}{P198}
\lookupPut{R_2uVVFWYUk1C2HUy}{P199}
\lookupPut{R_1JVoFjMj9hRe341}{P200}
\lookupPut{R_1jU71U36uDIk9M1}{P201}
\lookupPut{R_2WP8oE68QOuHpK0}{P202}
\lookupPut{R_1i57qSQQQ9YVS0E}{P203}
\lookupPut{R_BDGu0J5G2nvhVqV}{P204}
\lookupPut{R_3ndulyIO6ezZ7F0}{P205}
\lookupPut{R_1hQn66nd28LuU7J}{P206}
\lookupPut{R_1GAZRXr4im4JJ8g}{P207}
\lookupPut{R_1GZWlAawkNv67te}{P208}
\lookupPut{R_VV9GEsDKY9lmivD}{P209}
\lookupPut{R_2VfgoP3WwcacFvj}{P210}
\lookupPut{R_6QKyIp4jLgEbUOd}{P211}
\lookupPut{R_1cSpYEwFKia3jXr}{P212}
\lookupPut{R_1jeRGdfFPfN4QKo}{P213}
\lookupPut{R_1Lo0SFcJ44LqSNH}{P214}
\lookupPut{R_2uUuFUOqStFMQ5A}{P215}
\lookupPut{R_Dw8zz6MuLmsxwOt}{P216}
\lookupPut{R_3qqhUY1Tw1rwJoQ}{P217}
\lookupPut{R_2Yy0OVf6eCqk5QG}{P218}
\lookupPut{R_1jGOWxA8OuWHPpU}{P219}
\lookupPut{R_1f753RSW2En1otL}{P220}
\lookupPut{R_07BN0jQmksvASWZ}{P221}
\lookupPut{R_1kZwoRM2eXtelYx}{P222}
\lookupPut{R_XRg5AHlHyQ3FWWl}{P223}
\lookupPut{R_DCWefOgp6Jq0VmV}{P224}
\lookupPut{R_3QXY7xZpkyAH0PR}{P225}
\lookupPut{R_RDh7jD7qdNqtQjL}{P226}
\lookupPut{R_25YoTBxKvG4K6d0}{P227}
\lookupPut{R_1LpwxqHcsPZkN7T}{P228}
\lookupPut{R_2dyAqPg5KvAlZ9v}{P229}
\lookupPut{R_88S9TN4Yaol2mCB}{P230}
\lookupPut{R_YQyW9vQH2vJlGTL}{P231}
\lookupPut{R_PON27M1uVYkkOGt}{P232}
\lookupPut{R_2VF1WJpXALrdgcY}{P233}
\lookupPut{R_2whLDSv9SbTUF5G}{P234}
\lookupPut{R_3oyGHBR9o42ijPK}{P235}
\lookupPut{R_1i2qAnjmkAPWPGx}{P236}
\lookupPut{R_1oFuXaIUG4okhni}{P237}
\lookupPut{R_1Ea1jZ3akwXiHvm}{P238}
\lookupPut{R_1IK2VRbEXRYw7tF}{P239}
\lookupPut{R_3lVQNviDxGqsayr}{P240}
\lookupPut{R_26nWsKfGvqDa7K0}{P241}
\lookupPut{R_1DPbQEYvfZkQ0zT}{P242}
\lookupPut{R_yNNmtIm4a6IaAff}{P243}
\lookupPut{R_3PnmkcpUtz4Gan4}{P244}
\lookupPut{R_ZfWt9MAc6W0294B}{P245}
\lookupPut{R_12MtimXY6PrQmc5}{P246}
\lookupPut{R_08pWI5oE0ZrgJtD}{P247}
\lookupPut{R_3CAW1Go6RAsg8bL}{P248}
\lookupPut{R_3Do2Z6u2qjT4fzS}{P249}
\lookupPut{R_2dGi33jmjhpDwg4}{P250}
\lookupPut{R_12mOZwZceS8Yk1Q}{P251}
\lookupPut{R_3dKRkKkR5UNk4pv}{P252}
\lookupPut{R_000uROwCEp1gak1}{P253}
\lookupPut{R_AFYhYr8LQ7hDK13}{P254}
\lookupPut{R_OecvUDTZy6LgWsh}{P255}
\lookupPut{R_24i3iv4T5kzUyDd}{P256}
\lookupPut{R_8GlNbg5yOnHPfDb}{P257}
\lookupPut{R_1P7W7TbUUqJIzO8}{P258}
\lookupPut{R_2zYpwJVfpHd5sOY}{P259}
\lookupPut{R_3m2nyI5kj0cyZmE}{P260}
\lookupPut{R_ZKPbLZWN7ATxK6t}{P261}
\lookupPut{R_325WMTapBP4nBlS}{P262}
\lookupPut{R_s4BxrsKJmaRHtOF}{P263}
\lookupPut{R_2ye0rXuSksXIycZ}{P264}
\lookupPut{R_3HzdtsvZn3iPd6P}{P265}
\lookupPut{R_pbZhz9PC1PBuqAh}{P266}
\lookupPut{R_3Dqd6huO1qTyftd}{P267}
\lookupPut{R_3h3znVOEsmD8uWK}{P268}
\lookupPut{R_RyrN6MIqJ19FyLv}{P269}
\lookupPut{R_1E40USJYRn54NO5}{P270}
\lookupPut{R_3q8MDfaym6LAJSB}{P271}
\lookupPut{R_2qaWuYdeenywn46}{P272}
\lookupPut{R_262vUuwGEKcmaAs}{P273}
\lookupPut{R_5BkOn841VrHBS2R}{P274}
\lookupPut{R_27Ws38XjQcRiJjJ}{P275}
\lookupPut{R_1Eiyu74sOICpYE3}{P276}
\lookupPut{R_3KSKnIlnNFB6n26}{P277}
\lookupPut{R_1Kj9foggw0JIKyG}{P278}
\lookupPut{R_2CIWPMb8laoVsC8}{P279}
\lookupPut{R_2sXzrd0cwIX7JOo}{P280}
\lookupPut{R_2BsQneZu6Tq6hPq}{P281}
\lookupPut{R_3gZdfNwmRd8ieOt}{P282}
\lookupPut{R_2eQdGdvA0owE1si}{P283}
\lookupPut{R_2cioupPEFARrY1v}{P284}
\lookupPut{R_sNb9fjxBC3N93oJ}{P285}
\lookupPut{R_3kdAvlJLof42Ksk}{P286}
\lookupPut{R_2417U4xOSCvjinM}{P287}
\lookupPut{R_2P0saHapEZlXMAp}{P288}
\lookupPut{R_2v1FxwSFcqU4Ycm}{P289}
\lookupPut{R_QfwWXf0lt7LmSTD}{P290}
\lookupPut{R_1pmTy550R0e89iK}{P291}
\lookupPut{R_2zCFYEsfhQTdaMa}{P292}
\lookupPut{R_2644hYXudJKHbDX}{P293}
\lookupPut{R_2v2jjJgDlspVBFB}{P294}
\lookupPut{R_VWhRr8CXRQJtix3}{P295}
\lookupPut{R_1d6yAdZ9nxYMGrS}{P296}
\lookupPut{R_24eKyezJqZa6kSM}{P297}
\lookupPut{R_2D2KToeozIPJfTp}{P298}
\lookupPut{R_xa5Vxd9zIhmYmpH}{P299}
\lookupPut{R_sjOJmkAYd8NUuqt}{P300}
\lookupPut{R_1K9Ieb47xfXIOFA}{P301}
\lookupPut{R_1QlLDR7CbzaIClT}{P302}
\lookupPut{R_vGeFHoBvEHbRo7T}{P303}
\lookupPut{R_1rla0ACgvIzd7ud}{P304}
\lookupPut{R_33pXZtOQBd4jvQO}{P305}
\lookupPut{R_37Ot1e2qd26n7Ql}{P306}
\lookupPut{R_2pRhpuvbKXeTlTM}{P307}
\lookupPut{R_2SB8eHRch2Q03hb}{P308}
\lookupPut{R_3O97NV84zib4Ja3}{P309}
\lookupPut{R_2uBurgdnvRZrOl7}{P310}
\lookupPut{R_3kFGw0LoPy0Er37}{P311}
\lookupPut{R_3e9ABojvWPnVeT6}{P312}
\lookupPut{R_XKVInljoQGRM5QR}{P313}
\lookupPut{R_2cct4FkeO5snjvy}{P314}
\lookupPut{R_eEaWtQPjV4ObGQF}{P315}
\lookupPut{R_bfiMMsOGzMNk0OB}{P316}
\lookupPut{R_2QPoojNVJ45811t}{P317}
\lookupPut{R_3ET1d0UhA7jFj6J}{P318}
\lookupPut{R_Z2es3UtvbnMk4HT}{P319}
\lookupPut{R_AEsMx2C8PJI7Y3v}{P320}
\lookupPut{R_2D2C8mtf1Y0a6JA}{P321}
\lookupPut{R_2gdEJvSSwh0sm8F}{P322}
\lookupPut{R_12KXlYxiSoW3ujx}{P323}
\lookupPut{R_3oQRWS3qjv9OZeb}{P324}
\lookupPut{R_3ni8NhfSg4sPG5V}{P325}
\lookupPut{R_1Q4qlB818xh1DPU}{P326}
\lookupPut{R_WjrMn5zjiG5Wyjf}{P327}
\lookupPut{R_1Du55rJNEfh192R}{P328}
\lookupPut{R_Ce6WM4ItvLS4wud}{P329}
\lookupPut{R_3g4S2bScIDPd5cC}{P330}
\lookupPut{R_9p44ifS8ov7d2dr}{P331}
\lookupPut{R_24qNSh1WgZUZIi6}{P332}
\lookupPut{R_3Msp438LwQPIJ6G}{P333}
\lookupPut{R_6KXj3scqzInDwXL}{P334}
\lookupPut{R_3G2gNb061Igq53H}{P335}
\lookupPut{R_wWPeUvchjivuJfr}{P336}
\lookupPut{R_1jdIgZ4CnxcuzEI}{P337}
\lookupPut{R_sSa5knrOmMfAFep}{P338}
\lookupPut{R_1HbjXQwQZjLlLyY}{P339}
\lookupPut{R_2ZUIohkJyAgtRTH}{P340}
\lookupPut{R_1qWiANlGWTR4AdF}{P341}
\lookupPut{R_VPt13bW4hwXJpLz}{P342}
\lookupPut{R_33d05EkJHhmiu9x}{P343}
\lookupPut{R_3e3TiM18jbs4Y8h}{P344}
\lookupPut{R_SDzTK98b5XqflHH}{P345}
\lookupPut{R_1DvYJW1TpJkRoBJ}{P346}
\lookupPut{R_eFY2g03hgWmwHlf}{P347}
\lookupPut{R_2PBTJGkqGDsQnpy}{P348}
\lookupPut{R_3FKEk65eiGg7XjF}{P349}
\lookupPut{R_3qsVVZm5K1JMW22}{P350}
\lookupPut{R_5j3YpYRyOajsS09}{P351}
\lookupPut{R_3F3urxl3PvDeqf3}{P352}
\lookupPut{R_3NJ5FXnVcA0hBYQ}{P353}
\lookupPut{R_2OPve2WLV3cRmq6}{P354}
\lookupPut{R_9Bs7nRCjqsNAGhX}{P355}
\lookupPut{R_1nPnp6OSuePrULQ}{P356}
\lookupPut{R_25u5cqheDLC9vmN}{P357}
\lookupPut{R_qL145eVuAPAcVNL}{P358}
\lookupPut{R_2rr7wGOSO12cOpk}{P359}
\lookupPut{R_2QR1E89Xz5Z0S5E}{P360}
\lookupPut{R_3s0Ot8vax9OIQLg}{P361}
\lookupPut{R_06wEzdVzUeCwGjf}{P362}
\lookupPut{R_1GKtDME95om3hpY}{P363}
\lookupPut{R_305yallHEH6pC7g}{P364}
\lookupPut{R_3CQqwM1zWuaoolg}{P365}
\lookupPut{R_2s70cz0zKOVs8bG}{P366}
\lookupPut{R_3r1eBHhKz3Dw8MD}{P367}
\lookupPut{R_1KeFcVqrEB6uXjj}{P368}
\lookupPut{R_3je7a0Iot4QcYEc}{P369}
\lookupPut{R_10wmOY99YAsdGZa}{P370}
\lookupPut{R_udH3Z6mtJqScm6B}{P371}
\lookupPut{R_3MaLK1gXm0TYupS}{P372}
\lookupPut{R_2B4JDwte3OQIvS1}{P373}
\lookupPut{R_3sIRiyHCG93X1bb}{P374}
\lookupPut{R_2TB0gto6I21FAqp}{P375}
\lookupPut{R_3EXcnCS9fTCGVnY}{P376}
\lookupPut{R_1Cj2OjlSPDhz16B}{P377}
\lookupPut{R_1n2b7HNMPZfePlk}{P378}
\lookupPut{R_1JOPBIWBjxKdYzw}{P379}
\lookupPut{R_1eEsJvgnLUqlJjw}{P380}
\lookupPut{R_28ODSruCNh9fKOm}{P381}
\lookupPut{R_sGBhdNGbuVb0O0p}{P382}
\lookupPut{R_3Dw1GzmccLKKTg0}{P383}
\lookupPut{R_30pYJO3WEDuRcyZ}{P384}
\lookupPut{R_3q9JbDFiipQqm1U}{P385}
\lookupPut{R_33EIYrrAkfXsTas}{P386}
\lookupPut{R_2akORkJlDRkR50o}{P387}
\lookupPut{R_2VOwXRakF21RM0j}{P388}
\lookupPut{R_D2IXYhe8AmAeJQl}{P389}
\lookupPut{R_1IvnY3HqBnQdn2a}{P390}
\lookupPut{R_ZFbIaOn67W1YBG1}{P391}
\lookupPut{R_1OiCm1p9ZMjaqsp}{P392}
\lookupPut{R_dp1qxmsFs96NeRH}{P393}
\lookupPut{R_3qyuC1g55j9X1Gs}{P394}
\lookupPut{R_3r1aetU6fCRdS2E}{P395}
\lookupPut{R_qQ7epZr2st7O4pj}{P396}
\lookupPut{R_3szUM8uwBdfAplf}{P397}
\lookupPut{R_3lWfRGeuQNl7JH4}{P398}
\lookupPut{R_ZjBQyHWxjB4sEZb}{P399}
\lookupPut{R_5sAML4XQpiaOkxj}{P400}
\lookupPut{R_TtSRu3DUbIy2Vy1}{P401}
\lookupPut{R_3KDXeRGxundHddM}{P402}
\lookupPut{R_1jlfaCMQ4CSzNo6}{P403}
\lookupPut{R_Z36DdHieudInyFj}{P404}
\lookupPut{R_z2Ri4TFhWxAWLCN}{P405}
\lookupPut{R_1LcEyabCaCgDQXl}{P406}
\lookupPut{R_3nUwAjhGMbAI0Hw}{P407}
\lookupPut{R_bISKF0G94Jx1Lbz}{P408}
\lookupPut{R_20NCgjuw5UeW498}{P409}
\lookupPut{R_3jVRMs1aaXTNaNJ}{P410}
\lookupPut{R_9EL1nJJEs7VBwL7}{P411}
\lookupPut{R_1DwI97OLsXkUGJC}{P412}
\lookupPut{R_3hEgipfTL57jLSB}{P413}
\lookupPut{R_27Cokw74SBMS0Lt}{P414}
\lookupPut{R_1pKlunUbJR3ma9I}{P415}
\lookupPut{R_1pKYhkriiTPazwc}{P416}
\lookupPut{R_29vxy5iVHPopyQ7}{P417}
\lookupPut{R_3O9CpSwILvYbmdz}{P418}
\lookupPut{R_3emM8WbgPQvmkx2}{P419}
\lookupPut{R_2ck1OQMGOXhf8cg}{P420}
\lookupPut{R_271EUhrEdCnyVIy}{P421}
\lookupPut{R_31NmQe2M8DT7lAx}{P422}
\lookupPut{R_3Eg20ULxcxKiMNe}{P423}
\lookupPut{R_1rCv7KTGho0sdup}{P424}
\lookupPut{R_yDshnTOoiA0ZQPL}{P425}
\lookupPut{R_22VRzzZcTirOqw8}{P426}
\lookupPut{R_10SgfoX58CyXiF5}{P427}
\lookupPut{R_WDsnSMbepKFaudj}{P428}
\lookupPut{R_3qTAA9nhQ1nN2yi}{P429}
\lookupPut{R_tLqyU0sUUhYHMqt}{P430}
\lookupPut{R_2R9a9ekplXtPl3W}{P431}
\lookupPut{R_6QK10EorX7Z9lOp}{P432}
\lookupPut{R_3HTS3lfNSwaJxD5}{P433}
\lookupPut{R_egJW8N4f1SKaYAV}{P434}
\lookupPut{R_xEnlVPlTbp8Jx73}{P435}
\lookupPut{R_2SvFEqxb8E1hj0W}{P436}
\lookupPut{R_1LtBEWG8mCorpMW}{P437}
\lookupPut{R_2c0Fd2plrfTdphE}{P438}
\lookupPut{R_2xIXzt72SjeOQ8j}{P439}
\lookupPut{R_2aLhGLVW850Gr0q}{P440}
\lookupPut{R_3n62a0Xyt14glla}{P441}
\lookupPut{R_3338hUy45gMQSgc}{P442}
\lookupPut{R_1F4icNZHThwBCiu}{P443}
\lookupPut{R_Y9x8KqjffXzacqR}{P444}
\lookupPut{R_3LhAcg4T7zPUm7a}{P445}
\lookupPut{R_3dRMPZbprsfLjHZ}{P446}
\lookupPut{R_1FzgZQko4Tr8v6u}{P447}
\lookupPut{R_6ffF35ZhPd1P0T7}{P448}
\lookupPut{R_1Pd8DA5yHOADVio}{P449}
\lookupPut{R_2BreRClyOYNNgSB}{P450}
\lookupPut{R_2e3WlTH85A0tYye}{P451}
\lookupPut{R_1oce6XFJa8hxx4P}{P452}
\lookupPut{R_3KJSE776qtvAKoV}{P453}
\lookupPut{R_2CCmhAfEElwAszy}{P454}
\lookupPut{R_bNI3VIOmIqUvUu5}{P455}


==> lookup_questions.tex <==
\lookupPut{Q32}{Which of the following information about your skills would you display on GitHub to just yourself, your collaborators, and the public?}



\lookupPut{C3}{Do you understand and consent to these terms?}
\lookupPut{Q4_1}{Demographics and Background What is your gender? - Selected Choice - Woman}
\lookupPut{Q4_2}{Demographics and Background What is your gender? - Selected Choice - Man}
\lookupPut{Q4_3}{Demographics and Background What is your gender? - Selected Choice - Non-binary / gender diverse}
\lookupPut{Q4_4}{Demographics and Background What is your gender? - Selected Choice - Prefer to self-describe}
\lookupPut{Q4_5}{Demographics and Background What is your gender? - Selected Choice - Prefer not to answer}
\lookupPut{Q4_4_TEXT}{Demographics and Background What is your gender? - Prefer to self-describe - Text}
\lookupPut{Q5_1}{What is your ethnicity/origin you identify with (select all that apply)? - Selected Choice - White}
\lookupPut{Q5_2}{What is your ethnicity/origin you identify with (select all that apply)? - Selected Choice - Asian}
\lookupPut{Q5_3}{What is your ethnicity/origin you identify with (select all that apply)? - Selected Choice - Black or African}
\lookupPut{Q5_4}{What is your ethnicity/origin you identify with (select all that apply)? - Selected Choice - Hispanic or Latino}
\lookupPut{Q5_5}{What is your ethnicity/origin you identify with (select all that apply)? - Selected Choice - Middle Eastern}
\lookupPut{Q5_6}{What is your ethnicity/origin you identify with (select all that apply)? - Selected Choice - American Indian or Alaska Native}
\lookupPut{Q5_7}{What is your ethnicity/origin you identify with (select all that apply)? - Selected Choice - Native American or Other Pacific Islander}
\lookupPut{Q5_8}{What is your ethnicity/origin you identify with (select all that apply)? - Selected Choice - Other (please specify)}
\lookupPut{Q5_9}{What is your ethnicity/origin you identify with (select all that apply)? - Selected Choice - Prefer not to report}
\lookupPut{Q5_8_TEXT}{What is your ethnicity/origin you identify with (select all that apply)? - Other (please specify) - Text}
\lookupPut{Q6}{How many OSS projects have you worked on (give your best estimation)?}
\lookupPut{Q7_1}{Currently, what are your roles in the OSS projects you are most active in? - Selected Choice - Documentation writer}
\lookupPut{Q7_2}{Currently, what are your roles in the OSS projects you are most active in? - Selected Choice - Bug submitter}
\lookupPut{Q7_3}{Currently, what are your roles in the OSS projects you are most active in? - Selected Choice - Graphic artist}
\lookupPut{Q7_4}{Currently, what are your roles in the OSS projects you are most active in? - Selected Choice - Translator}
\lookupPut{Q7_5}{Currently, what are your roles in the OSS projects you are most active in? - Selected Choice - Coder}
\lookupPut{Q7_6}{Currently, what are your roles in the OSS projects you are most active in? - Selected Choice - Maintainer}
\lookupPut{Q7_7}{Currently, what are your roles in the OSS projects you are most active in? - Selected Choice - Porter}
\lookupPut{Q7_8}{Currently, what are your roles in the OSS projects you are most active in? - Selected Choice - Tool builder}
\lookupPut{Q7_9}{Currently, what are your roles in the OSS projects you are most active in? - Selected Choice - GUI designer}
\lookupPut{Q7_10}{Currently, what are your roles in the OSS projects you are most active in? - Selected Choice - Other (please specify)}
\lookupPut{Q7_10_TEXT}{Currently, what are your roles in the OSS projects you are most active in? - Other (please specify) - Text}
\lookupPut{Q8}{OSS projects for social good are projects where the outcome distinctly targets a community of people to overcome a societal issue.Do you think all OSS projects are for social good?}
\lookupPut{Q9}{Have you worked on an OSS project that is for social good?}
\lookupPut{Q10}{How do you define skills in the context of OSS? What are some examples of such skills?}
\lookupPut{Q11}{What are your strategies to grow your skills in the context of OSS?}
\lookupPut{Q12}{Do you use GitHub to display skills and experiences that are relevant for OSS development?}
\lookupPut{Q13_1}{How do you display your skills and experiences that are relevant for OSS development on GitHub? - Selected Choice - GitHub profile description}
\lookupPut{Q13_2}{How do you display your skills and experiences that are relevant for OSS development on GitHub? - Selected Choice - Actively contributing to OSS projects}
\lookupPut{Q13_3}{How do you display your skills and experiences that are relevant for OSS development on GitHub? - Selected Choice - Having public repositories}
\lookupPut{Q13_4}{How do you display your skills and experiences that are relevant for OSS development on GitHub? - Selected Choice - Linking social media accounts to GitHub profile}
\lookupPut{Q13_5}{How do you display your skills and experiences that are relevant for OSS development on GitHub? - Selected Choice - Linking personal website to GitHub profile}
\lookupPut{Q13_6}{How do you display your skills and experiences that are relevant for OSS development on GitHub? - Selected Choice - Other (please specify)}
\lookupPut{Q13_6_TEXT}{How do you display your skills and experiences that are relevant for OSS development on GitHub? - Other (please specify) - Text}
\lookupPut{Q14}{Do you use LinkedIn to display skills and experiences that are relevant for OSS development?}
\lookupPut{Q15_1}{How do you display skills and experiences that are relevant for OSS development on LinkedIn? - Selected Choice - LinkedIn experiences}
\lookupPut{Q15_2}{How do you display skills and experiences that are relevant for OSS development on LinkedIn? - Selected Choice - Descriptions to LinkedIn experiences}
\lookupPut{Q15_3}{How do you display skills and experiences that are relevant for OSS development on LinkedIn? - Selected Choice - Skills}
\lookupPut{Q15_4}{How do you display skills and experiences that are relevant for OSS development on LinkedIn? - Selected Choice - Endorsements on skills}
\lookupPut{Q15_5}{How do you display skills and experiences that are relevant for OSS development on LinkedIn? - Selected Choice - Skill quizzes}
\lookupPut{Q15_6}{How do you display skills and experiences that are relevant for OSS development on LinkedIn? - Selected Choice - Recommendations from colleagues}
\lookupPut{Q15_7}{How do you display skills and experiences that are relevant for OSS development on LinkedIn? - Selected Choice - Honors and awards}
\lookupPut{Q15_8}{How do you display skills and experiences that are relevant for OSS development on LinkedIn? - Selected Choice - Courses}
\lookupPut{Q15_9}{How do you display skills and experiences that are relevant for OSS development on LinkedIn? - Selected Choice - Projects}
\lookupPut{Q15_10}{How do you display skills and experiences that are relevant for OSS development on LinkedIn? - Selected Choice - Other (please specify)}
\lookupPut{Q15_10_TEXT}{How do you display skills and experiences that are relevant for OSS development on LinkedIn? - Other (please specify) - Text}
\lookupPut{Q16_1}{Rate the following skills based on their importance for OSS projects. - Teaches others to be involved in the OSS project}
\lookupPut{Q16_2}{Rate the following skills based on their importance for OSS projects. - Has commitment to the OSS project}
\lookupPut{Q16_3}{Rate the following skills based on their importance for OSS projects. - Has experience with specific tools, frameworks, or programming languages}
\lookupPut{Q16_4}{Rate the following skills based on their importance for OSS projects. - Has strong problem-solving skills}
\lookupPut{Q16_5}{Rate the following skills based on their importance for OSS projects. - Is familiar with OSS practices}
\lookupPut{Q16_6}{Rate the following skills based on their importance for OSS projects. - Puts in effort to make high-quality contributions}
\lookupPut{Q16_7}{Rate the following skills based on their importance for OSS projects. - Is a strong communicator}
\lookupPut{Q16_8}{Rate the following skills based on their importance for OSS projects. - Learns continuously}
\lookupPut{Q16_9}{Rate the following skills based on their importance for OSS projects. - Follows proper processes to make contributions to OSS projects}
\lookupPut{Q16_10}{Rate the following skills based on their importance for OSS projects. - Is a strong project manager}
\lookupPut{Q16_11}{Rate the following skills based on their importance for OSS projects. - Builds good relationships with stakeholders}
\lookupPut{Q16_12}{Rate the following skills based on their importance for OSS projects. - Has knowledge of algorithms, data structures, and programming paradigms}
\lookupPut{Q16_13}{Rate the following skills based on their importance for OSS projects. - Is available to answer questions}
\lookupPut{Q17_1}{Rate the following skills based on their importance for OSS projects that are for social good.OSS projects for social good are projects where the outcome distinctly targets a community of people to overcome a societal issue. - Teaches others to be involved in the OSS project}
\lookupPut{Q17_2}{Rate the following skills based on their importance for OSS projects that are for social good.OSS projects for social good are projects where the outcome distinctly targets a community of people to overcome a societal issue. - Has commitment to the OSS project}
\lookupPut{Q17_3}{Rate the following skills based on their importance for OSS projects that are for social good.OSS projects for social good are projects where the outcome distinctly targets a community of people to overcome a societal issue. - Has experience with specific tools, frameworks, or programming languages}
\lookupPut{Q17_4}{Rate the following skills based on their importance for OSS projects that are for social good.OSS projects for social good are projects where the outcome distinctly targets a community of people to overcome a societal issue. - Has strong problem-solving skills}
\lookupPut{Q17_5}{Rate the following skills based on their importance for OSS projects that are for social good.OSS projects for social good are projects where the outcome distinctly targets a community of people to overcome a societal issue. - Is familiar with OSS practices}
\lookupPut{Q17_6}{Rate the following skills based on their importance for OSS projects that are for social good.OSS projects for social good are projects where the outcome distinctly targets a community of people to overcome a societal issue. - Puts in effort to make high-quality contributions}
\lookupPut{Q17_7}{Rate the following skills based on their importance for OSS projects that are for social good.OSS projects for social good are projects where the outcome distinctly targets a community of people to overcome a societal issue. - Is a strong communicator}
\lookupPut{Q17_8}{Rate the following skills based on their importance for OSS projects that are for social good.OSS projects for social good are projects where the outcome distinctly targets a community of people to overcome a societal issue. - Learns continuously}
\lookupPut{Q17_9}{Rate the following skills based on their importance for OSS projects that are for social good.OSS projects for social good are projects where the outcome distinctly targets a community of people to overcome a societal issue. - Follows proper processes to make contributions to OSS projects}
\lookupPut{Q17_10}{Rate the following skills based on their importance for OSS projects that are for social good.OSS projects for social good are projects where the outcome distinctly targets a community of people to overcome a societal issue. - Is a strong project manager}
\lookupPut{Q17_11}{Rate the following skills based on their importance for OSS projects that are for social good.OSS projects for social good are projects where the outcome distinctly targets a community of people to overcome a societal issue. - Builds good relationships with stakeholders}
\lookupPut{Q17_12}{Rate the following skills based on their importance for OSS projects that are for social good.OSS projects for social good are projects where the outcome distinctly targets a community of people to overcome a societal issue. - Has knowledge of algorithms, data structures, and programming paradigms}
\lookupPut{Q17_13}{Rate the following skills based on their importance for OSS projects that are for social good.OSS projects for social good are projects where the outcome distinctly targets a community of people to overcome a societal issue. - Is available to answer questions}
\lookupPut{Q18}{List any skills not included in the questions above that you would display on your GitHub profile.}
\lookupPut{Q19_1}{Rate the following skills by how likely you are to improve them in the next 12 months. - Teaches others to be involved in the OSS project}
\lookupPut{Q19_2}{Rate the following skills by how likely you are to improve them in the next 12 months. - Has commitment to the OSS project}
\lookupPut{Q19_3}{Rate the following skills by how likely you are to improve them in the next 12 months. - Has experience with specific tools, frameworks, or programming languages}
\lookupPut{Q19_4}{Rate the following skills by how likely you are to improve them in the next 12 months. - Has strong problem-solving skills}
\lookupPut{Q19_5}{Rate the following skills by how likely you are to improve them in the next 12 months. - Is familiar with OSS practices}
\lookupPut{Q19_6}{Rate the following skills by how likely you are to improve them in the next 12 months. - Puts in effort to make high-quality contributions}
\lookupPut{Q19_7}{Rate the following skills by how likely you are to improve them in the next 12 months. - Is a strong communicator}
\lookupPut{Q19_8}{Rate the following skills by how likely you are to improve them in the next 12 months. - Learns continuously}
\lookupPut{Q19_9}{Rate the following skills by how likely you are to improve them in the next 12 months. - Follows proper processes to make contributions to OSS projects}
\lookupPut{Q19_10}{Rate the following skills by how likely you are to improve them in the next 12 months. - Is a strong project manager}
\lookupPut{Q19_11}{Rate the following skills by how likely you are to improve them in the next 12 months. - Builds good relationships with stakeholders}
\lookupPut{Q19_12}{Rate the following skills by how likely you are to improve them in the next 12 months. - Has knowledge of algorithms, data structures, and programming paradigms}
\lookupPut{Q19_13}{Rate the following skills by how likely you are to improve them in the next 12 months. - Is available to answer questions}
\lookupPut{Q20}{What factors influence which skills you want to improve on?}
\lookupPut{Q21_1}{Please rate your agreement with each of the following statements: - I know how to improve the OSS-related skills I want to grow.}
\lookupPut{Q21_2}{Please rate your agreement with each of the following statements: - I am taking steps to improve the OSS-related skills I want to grow.}
\lookupPut{Q21_3}{Please rate your agreement with each of the following statements: - I would be more motivated to improve my OSS-related skills if they were displayed publicly on GitHub.}
\lookupPut{Q22_1}{Please rate your agreement with each of the following statements: - I choose to contribute to an OSS project based on the skills that I can gain from the project.}
\lookupPut{Q22_2}{Please rate your agreement with each of the following statements: - I choose to contribute to an OSS project based on the skills that I can offer to the project.}
\lookupPut{Q22_3}{Please rate your agreement with each of the following statements: - I would choose to contribute to a project if I knew it had a collaborator who was strong at a particular skill.}
\lookupPut{Q22_4}{Please rate your agreement with each of the following statements: - I would choose to contribute to a project if I knew they were looking for contributors with a skill I have.}
\lookupPut{Q23_1}{For the OSS project(s) you maintain, rate the following skills based on how important they are for new contributors to have. - Teaches others to be involved in the OSS project}
\lookupPut{Q23_2}{For the OSS project(s) you maintain, rate the following skills based on how important they are for new contributors to have. - Has commitment to the OSS project}
\lookupPut{Q23_3}{For the OSS project(s) you maintain, rate the following skills based on how important they are for new contributors to have. - Has experience with specific tools, frameworks, or programming languages}
\lookupPut{Q23_4}{For the OSS project(s) you maintain, rate the following skills based on how important they are for new contributors to have. - Has strong problem-solving skills}
\lookupPut{Q23_5}{For the OSS project(s) you maintain, rate the following skills based on how important they are for new contributors to have. - Is familiar with OSS practices}
\lookupPut{Q23_6}{For the OSS project(s) you maintain, rate the following skills based on how important they are for new contributors to have. - Puts in effort to make high-quality contributions}
\lookupPut{Q23_7}{For the OSS project(s) you maintain, rate the following skills based on how important they are for new contributors to have. - Is a strong communicator}
\lookupPut{Q23_8}{For the OSS project(s) you maintain, rate the following skills based on how important they are for new contributors to have. - Learns continuously}
\lookupPut{Q23_9}{For the OSS project(s) you maintain, rate the following skills based on how important they are for new contributors to have. - Follows proper processes to make contributions to OSS projects}
\lookupPut{Q23_10}{For the OSS project(s) you maintain, rate the following skills based on how important they are for new contributors to have. - Is a strong project manager}
\lookupPut{Q23_11}{For the OSS project(s) you maintain, rate the following skills based on how important they are for new contributors to have. - Builds good relationships with stakeholders}
\lookupPut{Q23_12}{For the OSS project(s) you maintain, rate the following skills based on how important they are for new contributors to have. - Has knowledge of algorithms, data structures, and programming paradigms}
\lookupPut{Q23_13}{For the OSS project(s) you maintain, rate the following skills based on how important they are for new contributors to have. - Is available to answer questions}
\lookupPut{Q24}{As a maintainer, do you use GitHub to determine what skills a potential contributor has?}
\lookupPut{Q25_1}{As a maintainer, what do you use to determine what skills a potential contributor has? - Selected Choice - Public GitHub activity}
\lookupPut{Q25_2}{As a maintainer, what do you use to determine what skills a potential contributor has? - Selected Choice - Activity on social media platforms}
\lookupPut{Q25_3}{As a maintainer, what do you use to determine what skills a potential contributor has? - Selected Choice - Personal website}
\lookupPut{Q25_4}{As a maintainer, what do you use to determine what skills a potential contributor has? - Selected Choice - Public repositories the contributor owns}
\lookupPut{Q25_5}{As a maintainer, what do you use to determine what skills a potential contributor has? - Selected Choice - Contributions from contributor on your OSS project}
\lookupPut{Q25_6}{As a maintainer, what do you use to determine what skills a potential contributor has? - Selected Choice - Interactions with the potential contributor on your OSS project}
\lookupPut{Q25_7}{As a maintainer, what do you use to determine what skills a potential contributor has? - Selected Choice - Contributions from contributor on other OSS projects}
\lookupPut{Q25_8}{As a maintainer, what do you use to determine what skills a potential contributor has? - Selected Choice - Interactions with the potential contributor on other OSS projects}
\lookupPut{Q25_9}{As a maintainer, what do you use to determine what skills a potential contributor has? - Selected Choice - Other (please specify)}
\lookupPut{Q25_9_TEXT}{As a maintainer, what do you use to determine what skills a potential contributor has? - Other (please specify) - Text}
\lookupPut{Q27}{Consider the feature that shows contributor skills in the outlined red box. Rate your agreement with the following statement: I would like this feature on GitHub.}
\lookupPut{Q28}{Consider the feature that shows contributor skills and their ratings below in the outlined red box. Rate your agreement with the following statement: I would like this feature on GitHub.}
\lookupPut{Q29}{Consider the feature that shows contributor skills and their ratings below in the outlined red box. Rate your agreement with the following statement: I would like this feature on GitHub.}
\lookupPut{Q30}{Consider the feature that shows activities completed that are associated with the skill below in the outlined red box. Rate your agreement with the following statement: I would like this feature on GitHub.}
\lookupPut{Q31}{Consider the feature that shows how to improve contributor skills below. Rate your agreement with the following statement: I would like this feature on GitHub.}
\lookupPut{Q32_1}{Which of the following information about your skills would you display on GitHub to just yourself, your collaborators, and the public? - Skill name}
\lookupPut{Q32_2}{Which of the following information about your skills would you display on GitHub to just yourself, your collaborators, and the public? - Skill rating}
\lookupPut{Q32_3}{Which of the following information about your skills would you display on GitHub to just yourself, your collaborators, and the public? - Which activities you've done that correlate with the skill}
\lookupPut{Q32_4}{Which of the following information about your skills would you display on GitHub to just yourself, your collaborators, and the public? - Ways to improve the skill}
\lookupPut{Q33}{What motivates you to share skills information with others?}
\lookupPut{Q51}{Can you give examples of when it would be helpful to share skills information with others?}
\lookupPut{Q34_1}{Skill Ratings For each of the skills below, rate your agreement with the following statement: if I were proficient at this skill, I would publicly display that I have proficiency in this skill on my GitHub profile. - Team player}
\lookupPut{Q34_2}{Skill Ratings For each of the skills below, rate your agreement with the following statement: if I were proficient at this skill, I would publicly display that I have proficiency in this skill on my GitHub profile. - Commitment}
\lookupPut{Q34_3}{Skill Ratings For each of the skills below, rate your agreement with the following statement: if I were proficient at this skill, I would publicly display that I have proficiency in this skill on my GitHub profile. - Familiarity with open-source software}
\lookupPut{Q35_1}{For each of the programming languages below, rate your agreement with the following statement: if I were proficient at this programming language, I would publicly display that I have proficiency in this programming language on my GitHub profile. - JavaScript}
\lookupPut{Q35_2}{For each of the programming languages below, rate your agreement with the following statement: if I were proficient at this programming language, I would publicly display that I have proficiency in this programming language on my GitHub profile. - Python}
\lookupPut{Q35_3}{For each of the programming languages below, rate your agreement with the following statement: if I were proficient at this programming language, I would publicly display that I have proficiency in this programming language on my GitHub profile. - Java}
\lookupPut{Q35_4}{For each of the programming languages below, rate your agreement with the following statement: if I were proficient at this programming language, I would publicly display that I have proficiency in this programming language on my GitHub profile. - PHP}
\lookupPut{Q35_5}{For each of the programming languages below, rate your agreement with the following statement: if I were proficient at this programming language, I would publicly display that I have proficiency in this programming language on my GitHub profile. - C\#}
\lookupPut{Q35_6}{For each of the programming languages below, rate your agreement with the following statement: if I were proficient at this programming language, I would publicly display that I have proficiency in this programming language on my GitHub profile. - TypeScript}
\lookupPut{Q35_7}{For each of the programming languages below, rate your agreement with the following statement: if I were proficient at this programming language, I would publicly display that I have proficiency in this programming language on my GitHub profile. - Shell}
\lookupPut{Q35_8}{For each of the programming languages below, rate your agreement with the following statement: if I were proficient at this programming language, I would publicly display that I have proficiency in this programming language on my GitHub profile. - C}
\lookupPut{Q35_9}{For each of the programming languages below, rate your agreement with the following statement: if I were proficient at this programming language, I would publicly display that I have proficiency in this programming language on my GitHub profile. - Ruby}
\lookupPut{Q36}{Do you have any additional comments about skills in OSS? Is there anything else that you would like to share?}

==> utils.tex <==

\usepackage{geometry}

\usepackage{verbatim}

\usepackage{xspace}
\xspaceaddexceptions{]\}}


\usepackage{xcolor}
\usepackage{lscape}
\usepackage{colortbl}

\usepackage{microtype}

\usepackage{booktabs} %
\usepackage{makecell}
\usepackage{lipsum}
\usepackage[utf8]{inputenc}
\usepackage{array}
\usepackage{wrapfig}
\usepackage{multirow}
\usepackage{tabularx}
\usepackage{pifont}
\usepackage{lineno}
\usepackage{balance}
\usepackage{xcolor,pifont}
\newcommand{\cmark}{\text{\ding{51}}}
\newcommand{\xmark}{\text{\ding{55}}}
\usepackage{soul}
\newcommand{\rev}[1]{\textcolor{blue}{#1}}
\usepackage{balance}
\usepackage[linesnumbered, ruled,vlined]{algorithm2e}
\RequirePackage{pdflscape}
\usepackage{color}
\usepackage{setspace}
\usepackage{CJK}


\usepackage{flushend}
\usepackage{multicol}
\usepackage{placeins}
\usepackage{booktabs}
\usepackage{indentfirst}
\usepackage{fancybox}
\usepackage[most]{tcolorbox}
\usepackage{fontawesome}
\usepackage{mathtools}
\usepackage{MnSymbol,wasysym}
\usepackage{fontawesome}
\usepackage{rotating}
\usepackage{adjustbox}
\usepackage{colortbl}
\usepackage{color}
\usepackage{framed}
\definecolor{Gray}{gray}{0.9}
\definecolor{shadecolor}{gray}{0.95}
\usepackage{tikz}
\usetikzlibrary{trees,positioning,shapes,shadows,arrows}


\renewenvironment{quote}{%
   \list{}{%
     \rightmargin0cm
   }
   \item\relax
}
{\endlist}

\renewenvironment{quotation}{%
   \list{}{%
     \rightmargin0cm
   }
   \item\relax
}
{\endlist}

\usepackage{framed}
\usepackage[strict]{changepage}

\usepackage{lookup}
\include{lookup_participants}
\include{lookup_questions}

\usepackage{soul}

\definecolor{PAblue}{RGB}{0,122,204}%

\newcommand{\quo}[2]{ 
	\vspace{-0.15cm}
	\def\FrameCommand{%
		\hspace{0pt}%
		{\color{PAblue}\vrule width 2pt}%
		{\color{white}\vrule width 2pt}%
		\colorbox{white}
	}%
	\MakeFramed{\advance\hsize-\width\FrameRestore}%
	\noindent\hspace{-4.55pt}%
	\begin{adjustwidth}{}{0pt}
		\vspace{-2pt}%
		``\emph{#1}'' (\lookupGet{#2})
		\vspace{-3pt}
	\end{adjustwidth}\endMakeFramed%
	\vspace{-0.15cm}
}

\newcommand{\inlinequo}[2]{``\emph{#1}'' (\lookupGet{#2})}
\newcommand{\inlinequote}[1]{``\emph{#1}''}

\definecolor{boxcolor}{RGB}{238, 223, 204} %
\DeclareRobustCommand{\mybox}[2][gray!20]{%
\begin{tcolorbox}[   %
        breakable,
        left=0pt,
        right=0pt,
        top=0pt,
        bottom=0pt,
        colback=#1,
        colframe=black,
        width=\dimexpr\columnwidth\relax, 
        enlarge left by=0mm,
        boxsep=5pt,
        outer arc=4pt,
        boxrule=.5mm
        ]
        #2
\end{tcolorbox}
}


\newcommand{\questiontext}[1]{\lookupGet{#1}\xspace}

\usepackage{stackengine}

\definecolor{lightgreen}{RGB}{247,253,251}
\definecolor{newgreen}{RGB}{7,94,70}
\definecolor{bordergreen}{RGB}{101,223,190}

\newtcolorbox{myideabox}{sidebyside,
                         colback=lightgreen,
                         colframe=bordergreen, 
                         coltext=newgreen,
                         boxrule=0.9pt,
                         boxsep=5pt,
                         arc=1pt,
                         leftrule=0.8mm, 
                         lefthand width=0.4cm, 
                         lower separated=false, 
                         sidebyside gap=3mm, 
                                 right=1pt,
                            top=1pt,
        bottom=1pt,
                         left=3pt}

\DeclareRobustCommand{\anotherbox}[1]{%
\begin{myideabox}\centering\LARGE\faLightbulbO\tcblower
        #1
\end{myideabox}
}

\newcounter{bestpractice}%

\DeclareRobustCommand{\bestpracticebox}[1]{\refstepcounter{bestpractice}%
\begin{myideabox}\centering\LARGE\faLightbulbO\tcblower
\textbf{Best Practice \thebestpractice:} #1
\end{myideabox}
}











